Brain Biomarker Interpretation in ASD Using Deep Learning and fMRI

Autism spectrum disorder (ASD) is a complex neurodevelopmental disorder. Finding the biomarkers associated with ASD is extremely helpful to understand the underlying roots of the disorder and can lead to earlier diagnosis and more targeted treatment. Although Deep Neural Networks (DNNs) have been applied in functional magnetic resonance imaging (fMRI) to identify ASD, understanding the data-driven computational decision making procedure has not been previously explored. Therefore, in this work, we address the problem of interpreting reliable biomarkers associated with identifying ASD; specifically, we propose a 2-stage method that classifies ASD and control subjects using fMRI images and interprets the saliency features activated by the classifier. First, we trained an accurate DNN classifier. Then, for detecting the biomarkers, different from the DNN visualization works in computer vision, we take advantage of the anatomical structure of brain fMRI and develop a frequency-normalized sampling method to corrupt images. Furthermore, in the ASD vs. control subjects classification scenario, we provide a new approach to detect and characterize important brain features into three categories. The biomarkers we found by the proposed method are robust and consistent with previous findings in the literature. We also validate the detected biomarkers by neurological function decoding and comparing with the DNN activation maps.

==> matlab_history <==
%-- 09/26/2017 02:22:02 PM --%
a = 2
Generate_3DfMRI_dowmsampled
%-- 09/26/2017 09:25:50 PM --%
Generate_3DfMRI_dowmsampled
labels = MRIread([data_dir,'fsaverage/mri/',seg_name,'.mgz']);
%-- 10/10/2017 06:07:58 PM --%
idata = load_nifti('shen_2mm_268_parcellation.nii.gz');
a = idata.vol
idata = a
imsize = size(idata);
sz = [32 32 32];
h5create(['downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create(['downsample','.h5'],'/fMRI',[sz],'ChunkSize',[sz,1]);
h5create(['downsample','.h5'],'/fMRI',sz,'ChunkSize',[sz,1]);
h5create(['downsample','.h5'],'/fMRI',sz,'ChunkSize',sz);
[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:),1),sz(1)),linspace(1,size(idata(:,:,:),2),sz(2)),linspace(1,size(idata(:,:,:),3),sz(3)));
imout = interp3(idata,x,y,z);
h5write(['downsample','.h5'],'/fMRI',imout,[1,1,1],[sz,1]);
h5write(['downsample','.h5'],'/fMRI',imout,[1,1,1],sz);
%-- 10/10/2017 08:01:45 PM --%
idata = load_nifti('downsample.nii');
origim= nii_tool('img','silin.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.02 0.02])
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 300])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.02 0.02])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.02 0.02])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.01 0.01])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.1 0.1])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.005 0.005])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim,[32 32 1 32])),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.015])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.015])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image3.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image4.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image5.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image6.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image7.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(abs(newim),[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img2/image7.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[64 64 1 64]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img2/image7.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img2/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img2/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.03])
figure; montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.025])
origim= nii_tool('img','nii_img/image23.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image25.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image4.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image3.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img','nii_img/image23.nii');
newim= flipud(permute(origim,[2 3 1]));
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.025])
close all
imshow(newim[:,:,16])
imshow(newim(:,:,16))
imshow(newim(:,16,:))
imshow(newim(16,:,:))
imagesc(newim(16,:,:))
imagesc(squeeze(newim(16,:,:)))
figure;imagesc(squeeze(newim(:,16,:)))
origim= nii_tool('img','nii_img/image666.nii');
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img','nii_img/image16.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)))
origim= nii_tool('img','nii_img/image18.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)))
origim= nii_tool('img','nii_img/image9.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)))
figure;imagesc(squeeze(newim(:,16,:)),[0,0.03])
origim= nii_tool('img','nii_img/image3.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)))
figure;imagesc(squeeze(newim(:,16,:)),[0,0.025])
origim= nii_tool('img','nii_img/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)))
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.015])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.015])
origim= nii_tool('img','nii_img/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img/image31.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.018])
origim= nii_tool('img','nii_img/image22.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.018])
origim= nii_tool('img','nii_img/image14.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.018])
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img/image26.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img1_1/image26.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img1_1/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img1_1/image1.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.025])
origim= nii_tool('img','nii_img1_1/image24.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img1_1/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img1_1/image8.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img3_1/image8.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img3_1/image16.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img3_1/image0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img3_1/image11.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
origim= nii_tool('img','nii_img3_1/image14.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.025])
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
origim= nii_tool('img','nii_img3_1/image15.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
origim= nii_tool('img','nii_img3_1/image18.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
origim= nii_tool('img','nii_img3_1/image20.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
%-- 10/11/2017 09:44:55 PM --%
origim= nii_tool('img','output_oversub/con0.nii');
newim= flipud(permute(origim,[2 3 1]));
figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure; montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.025])
figure('position',[0,0,200,200]); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.025])
figure('position',[0,0,100,100]); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.025])
figure('position',[0,0,500,500]); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
figure('position',[0,0,5000,5000]); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
for i = 0:31
origim= nii_tool('img','output_oversub/con'+int2str(i)+'.nii');
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.02])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.02])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.02])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]))
end
close all
i = 0
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim-newim2,[16 16 1 16]))
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[0 0.01])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
end
i = 0
origim= nii_tool('img',strcat('output_oversub_o/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
i = 1
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
i = 3
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
i = 6
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.015])
close all
%-- 10/12/2017 12:13:25 PM --%
i =0
for i = 0:31
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.005])
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[0 0.01])
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.005])
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.008])
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.07])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.007])
i = 0
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[0 0.01])
close all
i =  166
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
i =10
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i =1
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
0
i = 0
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.02 0.02])
%-- 10/14/2017 05:17:17 PM --%
i = 10
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 0
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 3
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 4
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 5
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 6
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 7
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 8
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 9
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 10
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 11
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
12
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
NII_TOOL('save',reshape(newim-newim2,[16 16 1 16]),'mask.nii')
nii_tool('save',reshape(newim-newim2,[16 16 1 16]),'mask.nii')
nii=nii_tool('init',reshape(newim-newim2,[16 16 1 16]))
nii_tool('save',nii,'mask.nii')
nii=nii_tool('init',newim-newim2)
nii_tool('save',nii,'mask.nii')
a = newim-newim2
imshow(a(16,:,:))
imshow(squeeze(a(16,:,:)))
imshow(squeeze(a(8,:,:)))
imshow(squeeze(a(8,:,:)),[-0.001,0.001])
imshow(squeeze(a(8,:,:)),[-0.005,0.005])
imshow(squeeze(a(:,8,:)),[-0.005,0.005])
imshow(squeeze(a(:,:,8)),[-0.005,0.005])
imshow(squeeze(a(:,8,:)),[-0.005,0.005])
imshow(squeeze(a(2,:,:)),[-0.005,0.005])
imshow(squeeze(a(:,2,:)),[-0.005,0.005])
imshow(squeeze(a(:,8,:)),[-0.005,0.005])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
figure();imshow(squeeze(a(:,:,8)),[-0.005,0.005])
figure();plot(a(8,:,8))
figure();plot(a(:,8,8))
close all
sz=[109.91,91]
sz=[109,91,91]
[y,x,z]=ndgrid(linspace(1,size(a,1),sz(1)),linspace(1,size(a,2),sz(2)),linspace(1,size(a,3),sz(3)));
sout = interp3(sdata,x,y,z);
sout = interp3(a,x,y,z);
nii = nii_tool('load','silin.nii')
nii = nii_tool('load','shen_2mm_268_parcellation.nii')
nii = nii_tool('load','shen_2mm_268_parcellation.nii.gz')
b = permute(a,[2,1,3])
sz =[91,109,91]
[y,x,z]=ndgrid(linspace(1,size(b,1),sz(1)),linspace(1,size(b,2),sz(2)),linspace(1,size(sb,3),sz(3)));
sout = interp3(b,x,y,z);
[y,x,z]=ndgrid(linspace(1,size(b,1),sz(1)),linspace(1,size(b,2),sz(2)),linspace(1,size(b,3),sz(3)));
sout = interp3(b,x,y,z);
imshow(squeeze(b(:,:,45)))
imshow(squeeze(sout(:,:,45)))
imshow(squeeze(sout(:,:,45)),[-0.005,0.005])
figure(nii.img(:,:,45))
figure();imshow(nii.img(:,:,45))
figure();imshow(nii.img(:,45,:))
figure();imshow(squeeze(nii.img(:,45,:)))
imshow(squeeze(sout(:,45,:)),[-0.005,0.005])
figure();imshow(squeeze(nii.img(:,45,:)))
figure;imshow(squeeze(sout(:,45,:)),[-0.005,0.005])
figure;imshow(squeeze(sout(45,:,:)),[-0.005,0.005])
figure();imshow(squeeze(nii.img(45,:,:)))
c = imrotate3(sout,180,[0,0,1])
c = imrotate3(sout,180,[0,0,1]);
c = imrotate3(sout,180,[0,0,1],'linear');
c = imrotate3(sout,180,[0,0,1],'crop');
figure;imshow(squeeze(sout(c,:,:)),[-0.005,0.005])
figure;imshow(squeeze(c(45,:,:)),[-0.005,0.005])
figure;imshow(squeeze(c(:,45,:)),[-0.005,0.005])
figure;imshow(squeeze(c(:,:,45)),[-0.005,0.005])
c(c<0)=1
c(c>=0)=0;
nii=nii_tool('init',c)
nii_tool('save',nii,'mask.nii')
max(max(max(c)))
max(max(c))
imshow(c(:,45,:)
imshow(c(:,45,:))
imshow(c(:,:,45))
c
c = imrotate3(sout,180,[0,0,1],'crop');
min(min(min(c)))
pp = c >0;
nn = c <0;
c(pp) = 0
c(nn)=1;
max(max(max(c)))
nii=nii_tool('init',c)
nii_tool('save',nii,'mask.nii')
imshow(c(:,:,45))
c = imrotate3(sout,180,[0,0,1],'linear','crop');
imshow(c(:,:,45))
pp = c >0;
nn = c <0;
c(pp) = 0
c(nn)=1;
imshow(c(:,:,45))
c = imrotate3(sout,180,[0,0,1],'linear','crop');
nn = c <-0.002;
pp = c >= -0.002
c(pp) = 0
c(nn)=1;
imshow(c(:,:,45))
c = imrotate3(sout,180,[0,0,1],'linear','crop');
nn = c <-0.0015;
pp = c >= -0.0015;
c(pp) = 0;
c(nn)=1;
imshow(c(:,:,45))
nii=nii_tool('init',c)
nii_tool('save',nii,'mask.nii')
%-- 10/16/2017 09:51:13 AM --%
i =11
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
a = newim-newim2
b = permute(a,[2,1,3]);
[y,x,z]=ndgrid(linspace(1,size(b,1),sz(1)),linspace(1,size(b,2),sz(2)),linspace(1,size(b,3),sz(3)));
sz = [91,109,91];
[y,x,z]=ndgrid(linspace(1,size(b,1),sz(1)),linspace(1,size(b,2),sz(2)),linspace(1,size(b,3),sz(3)));
sout = interp3(b,x,y,z);
c = imrotate3(sout,180,[0,0,1],'crop');
doc imregister
altas = nii_tool('load','MNI152_T1_1mm_brain.nii.gz')
altas = nii_tool('load','MNI152_T1_2mm_brain.nii.gz')
[optimizer,metric]=imregconfig('monomodal');
movingRegistered = imregister(c, altas.img, 'affine', optimizer, metric);
nii = nii_tool('init',movingRegistered)
nii_tool('save',nii,'reg_diff.nii')
nii = nii_tool('init',c)
nii_tool('save',nii,'diff.nii')
%-- 10/19/2017 03:41:19 PM --%
% upsmaple image and correct coordinate
sdata = nii_tool('load','mask.nii').image;
sz=[91 109 91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sdata = nii_tool('load','mask.nii').image;
sdata = nii_tool('load','mask.nii')
sdata = nii_tool('load','mask.nii').img;
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
nii=nii_tool('init',sout);
nii_tool('save',nii,'mask_upsample.nii');
sout= permute(sout,[2 3 1])
nii=nii_tool('init',sout);
nii_tool('save',nii,'mask_upsample.nii');
snew = sout(abs(sout)>0.15)
snew = sout;
snew(abs(snew)<0.15)=0;
nii=nii_tool('init',snew);
nii_tool('save',nii,'mask_upsample_th0.15.nii');
snew= permute(snew,[2 1 3])
nii=nii_tool('init',snew);
nii_tool('save',nii,'mask_upsample_th0.15.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1])
snew = sout;
snew(abs(snew)<0.15)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',snew);
nii_tool('save',nii,'mask_upsample_84.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.1)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',snew);
nii_tool('save',nii,'mask_upsample_84_th0.1.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.1)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_th0.1.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.1)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_th0.13.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.13)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_th0.13.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','89.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
%snew(abs(snew)<0.13)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_89.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
%snew(abs(snew)<0.13)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_N_05.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.13)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_N_05_th0.13.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.15)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_N_05_th0.15.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.2)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_upsample_84_N_05_th0.2.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(snew<0.2)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_pos_upsample_84_N_05_th0.2.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(snew>-0.2)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_pos_upsample_84_N_05_th0.2.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(snew>-0.2)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_neg_upsample_84_N_05_th0.2.nii');
% upsmaple image and correct coordinate
sdata = nii_tool('load','84_N_05.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(snew<0.2)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask_pos_upsample_84_N_05_th0.2.nii');
upsampling
sdata = nii_tool('load','84_N_10.nii');
sdata = sdata.img;
sz=[91,109,91];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
sout= permute(sout,[2 3 1]);
snew = sout;
snew(abs(snew)<0.15)=0;
snew= permute(snew,[2 1 3]);
nii=nii_tool('init',-snew);
nii_tool('save',nii,'mask__upsample_84_N_10_th0.15.nii');
upsampling
avg_saliency
clear all
avg_saliency
upsampling
avg_saliency
max(max(img))
avg_saliency
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim+newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim+newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim+newim2,[16 16 1 16]),'displayrange',[-0.05 0.05])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(-newim+newim2,[16 16 1 16]),'displayrange',[-0.05 0.05])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(-newim+newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
colse all
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim1,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[0 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(-newim+newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim2,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('output_oversub_o2/con',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('output_oversub_o2/pat',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[-0.01 0.01])
end
close all
%-- 10/24/2017 05:59:42 PM --%
fMRI = nii_tool('img',"tfMRI-mean-reorient-brain-anat_flirt_6.nii.gz")
hdr = nii_tool('hdr',"tfMRI-mean-reorient-brain-anat_flirt_6.nii.gz")
hdr = nii_tool('hdr',"tfMRI-mean-reorient-brain-anat_flirt_6.nii")
fMRI = nii_tool('img',"tfMRI-mean-reorient-brain-anat_flirt_6.nii")
fMRI = nii_tool('img','tfMRI-mean-reorient-brain-anat_flirt_6.nii')
hdr = nii_tool('hdr','tfMRI-mean-reorient-brain-anat_flirt_6.nii');
fMRI = nii_tool('img','tfMRI-mean-reorient-brain-anat_flirt_6.nii');
fMRI = nii_tool('img','tfMRI-reorient-brain-mni152_2mm_fnirt.nii.gz');
size(fMRI)
imshow(fMRI(45,50,45,1)
imshow(fMRI(45,50,45,1))
imshow(fMRI(45,:,:,1))
imshow(squeeze(fMRI(45,:,:,1)))
imshow(squeeze(fMRI(:,:,45,1)))
imshow(squeeze(fMRI(:,45,:,1)))
imshow(imrotate(squeeze(fMRI(:,:,45,1),-90)))
imshow(imrotate(squeeze(fMRI(:,:,45,1)),-90))
making_video
imshow(imrotate(squeeze(fMRI(:,:,45,1)),-90),[-10000,10000])
max(max(max(fMRI)))
max(max(max(max(fMRI))))
min(min(min(min(fMRI))))
making_video
F = cell{3,1}
F(1) = im2frame(img)
img=double(imrotate(squeeze(fMRI(:,:,45,i)),-90)/(2.5000e+04));
F(1) = im2frame(img)
making_video
upsampling
%-- 10/30/2017 04:40:14 PM --%
upsampling
max(max(max(sdata)))
upsampling
max(max(max(sdata)))
upsampling
fMRI = nii_tool('load',aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz);
fMRI = nii_tool('load','aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz');
img = fMRI.img;
regions = [28,60,11109,11112,11116,11131,11137,12106,12107,12129,12138,12168,12170,12174];
len(regions)
length(regions)
color_mask
for i = 1:length(regions)
img==regions(i)
end
flag = 0
for i = 1:length(regions)
if sum(sum(img==regions(i)))>1
flag = flag +1
end
end
sum(sum(img==regions(i)))
flag = 0
for i = 1:length(regions)
if sum(sum(sum(img==regions(i))))>1
flag = flag +1
end
end
load('/media/xiaoxiao/Basket III/mri_server/MAT/labels.mat')
color_mask
a = hdf5read('community.h5')
a = hdf5read('community.h5','group1')
a = hdf5read('community.h5','/group1')
a = hdf5read('comunity.h5','/group1')
a = hdf5read('comunity.h5')
h5disp('comunity.h5')
a = hdf5read('comunity.h5','group1')
a.Data
group1=[11101,
11106,
11116,
11118,
11121,
11124,
11125,
11129,
11130,
11135,
11138,
11141,
11148,
11150,
11156,
11161,
11165,
11166,
11171,
11172,
11173,
11174,
12107,
12110,
12115,
12116,
12125,
12136,
12137,
12138,
12151,
12153,
12154,
12155,
12156,
12157,
12161,
12162,
12168,
12172,
12173,
12174
]
group2=[8,
47,
11101,
11102,
11105,
11106,
11107,
11111,
11112,
11113,
11114,
11115,
11116,
11118,
11119,
11120,
11121,
11122,
11125,
11126,
11127,
11128,
11136,
11139,
11140,
11143,
11145,
11148,
11152,
11153,
11154,
11155,
11157,
11158,
11159,
11160,
11162,
11163,
11165,
11166,
11168,
11169,
12102,
12111,
12116,
12119,
12120,
12121,
12122,
12125,
12126,
12127,
12130,
12137,
12138,
12143,
12145,
12151,
12152,
12157,
12158,
12159,
12160,
12161,
12162,
12166,
12173,
12174
]
group3=[10,
11,
12,
13,
17,
18,
26,
28,
49,
50,
51,
52,
53,
54,
58,
60,
11101,
11103,
11104,
11105,
11108,
11109,
11110,
11117,
11121,
11123,
11125,
11126,
11127,
11128,
11129,
11130,
11131,
11132,
11133,
11134,
11135,
11136,
11137,
11138,
11141,
11144,
11146,
11147,
11149,
11150,
11151,
11156,
11157,
11161,
11162,
11164,
11167,
11168,
11170,
11171,
11172,
11173,
11174,
11175,
12101,
12103,
12104,
12105,
12106,
12107,
12108,
12109,
12110,
12112,
12113,
12114,
12115,
12117,
12118,
12123,
12124,
12126,
12127,
12128,
12129,
12130,
12131,
12132,
12133,
12134,
12135,
12136,
12139,
12140,
12141,
12144,
12146,
12147,
12148,
12149,
12150,
12151,
12153,
12154,
12156,
12157,
12163,
12164,
12165,
12167,
12168,
12169,
12170,
12171,
12172,
12175
]
color_mask
group22=[8,
47,
11102,
11105,
11107,
11111,
11112,
11113,
11114,
11115,
11119,
11120,
11122,
11126,
11127,
11128,
11136,
11139,
11140,
11143,
11145,
11152,
11153,
11154,
11155,
11157,
11158,
11159,
11160,
11162,
11163,
11168,
11169,
12102,
12111,
12119,
12120,
12121,
12122,
12126,
12127,
12130,
12143,
12145,
12152,
12158,
12159,
12160,
12166
]
group33=[10,
11,
12,
13,
17,
18,
26,
28,
49,
50,
51,
52,
53,
54,
58,
60,
11103,
11104,
11108,
11109,
11110,
11117,
11123,
11131,
11132,
11133,
11134,
11137,
11144,
11146,
11147,
11149,
11151,
11164,
11167,
11170,
11175,
12101,
12103,
12104,
12105,
12106,
12108,
12109,
12112,
12113,
12114,
12117,
12118,
12123,
12124,
12128,
12129,
12131,
12132,
12133,
12134,
12135,
12139,
12140,
12141,
12144,
12146,
12147,
12148,
12149,
12150,
12163,
12164,
12165,
12167,
12169,
12170,
12171,
12175
]
color_mask
save('community/result1_2c.mat','group1','group22','group33')
g1 = 11105,
11117,
11124,
11127,
11128,
11129,
11139,
11157,
11165,
11166,
12106,
12113,
12120,
12125,
12126,
12127,
12143,
12148,
12151,
12157,
g1=[11105,
11117,
11124,
11127,
11128,
11129,
11139,
11157,
11165,
11166,
12106,
12113,
12120,
12125,
12126,
12127,
12143,
12148,
12151,
12157,
];
g2=[8,
47,
52,
11107,
11109,
11110,
11126,
11141,
11146,
11147,
11167,
11168,
11172,
11175,
12103,
12104,
12108,
12109,
12110,
12112,
12116,
12117,
12128,
12129,
12133,
12138,
12139,
12140,
12146,
12154,
12156,
12163,
12167,
12169,
12171,
12172,
12175
]
g3=[10,
11,
17,
18,
28,
49,
53,
54,
11101,
11102,
11106,
11111,
11112,
11113,
11114,
11119,
11120,
11121,
11122,
11125,
11131,
11132,
11134,
11135,
11137,
11138,
11143,
11144,
11145,
11148,
11149,
11150,
11152,
11153,
11154,
11155,
11158,
11159,
11160,
11162,
11163,
11169,
11170,
12101,
12102,
12105,
12107,
12111,
12114,
12119,
12121,
12122,
12123,
12124,
12131,
12135,
12137,
12141,
12144,
12145,
12149,
12152,
12153,
12158,
12159,
12160,
12161,
12165,
12166,
12170,
12173,
12174
];
color_mask
a = [ 0.68073447,  0.4266332 ,  0.28300809,  0.27411492,  0.26711573,
0.31581774,  0.2573941 ,  0.26777482,  0.31731752,  0.77920876,
0.38664009,  0.30758282,  0.30476435,  0.26801081,  0.27038971,
0.27122296,  0.27289445,  0.30348791,  0.26896067,  0.32088973,
0.33113261,  0.26010289,  0.26612938,  0.2786508 ,  0.2532586 ,
0.28313709,  0.30471644,  0.26497287,  0.36533457,  0.29815539,
0.27034138,  0.28168057,  0.36463798,  0.31563032,  0.25926853,
0.26491618,  0.34565219,  0.34527526,  0.25839408,  0.34853349,
0.26905145,  0.29315945,  0.2583108 ,  0.27569834,  0.28550389,
0.29411363,  0.24951663,  0.26978886,  0.27472982,  0.26924234,
0.24905187,  0.26388293,  0.26612186,  0.25472976,  0.24309546,
0.28164499,  0.26694163,  0.26575369,  0.25461245,  0.26643282,
0.29517922,  0.2734568 ,  0.30869822,  0.27565579,  0.25572203,
0.26795591,  0.25692835,  0.24722169,  0.26697611,  0.27224419,
0.29264875,  0.27661423,  0.29287848,  0.26828203,  0.22426316,
0.29300177,  0.2836459 ,  0.26852315,  0.2623078 ,  0.26618545,
0.26694331,  0.2767291 ,  0.27435639,  0.28764438,  0.27273544,
0.30901832,  0.27146178,  0.25164938,  0.26979815,  0.29419581,
0.26808723,  0.27009508,  0.25740181,  0.26958249,  0.28918682,
0.34328626,  0.2495939 ,  0.26993393,  0.28722332,  0.27490593,
0.30463911,  0.26625261,  0.24978517,  0.33739031,  0.28434855,
0.26747295,  0.27958867,  0.28993391,  0.30956487,  0.26585196,
0.27381101,  0.40476511,  0.39080263,  0.31191166,  0.37298397,
0.27338597,  0.34165782,  0.28578669,  0.23989933,  0.22771786,
0.26674657,  0.31528904,  0.22229265,  0.27790015,  0.2628542 ,
0.26491287,  0.27388439,  0.27267342,  0.26024642,  0.28815561,
0.26596945,  0.27107687,  0.26622961,  0.26155417,  0.26643282,
0.3123252 ,  0.30743836,  0.2978654 ,  0.27524605,  0.26639499,
0.27369244,  0.26616012,  0.2756297 ,  0.26750374,  0.27028045,
0.28360451,  0.27347192,  0.27681897,  0.26825031,  0.24271407,
0.28106445,  0.32370884,  0.28175257,  0.27074816,  0.27309468,
0.26655871,  0.2668119 ,  0.2843155 ,  0.27984344,  0.26270174,
0.25268391,  0.26775644,  0.26581804,  0.26863954,  0.27079988,
0.26397969,  0.25882925,  0.2651036 ]
a = label[122,
74,
119,
118,
149,
54,
67,
50,
46,
96,
102,
87,
160,
24,
58,
53,
64,
66,
6,
92,
42,
38,
166,
34,
21,
128,
133,
78,
159,
124,
51,
165,
125,
35,
27,
167,
57,
162,
109,
130,
52,
22,
141,
79,
132,
101,
139,
59,
134,
155,
120,
156,
56,
80,
68,
4,
105,
143,
161,
7,
65,
13,
90,
148,
73,
77,
163,
18,
40,
49,
93,
47,
88,
97,
91,
144,
30,
14,
153,
164,
131,
15,
86,
69,
127,
84,
16,
154,
115,
61,
146,
140,
110,
126,
3,
82,
48,
99,
138,
142,
63,
43,
71,
81,
147,
123,
23,
106,
158,
150,
55,
31,
152,
2,
25,
145,
76,
157,
104,
44,
117,
98,
83,
129,
94,
107,
70,
72,
75,
41,
45,
89,
60,
137,
29,
17,
100,
26,
12,
136,
11,
62,
85,
108,
113,
135,
121,
33,
5,
8,
19,
151,
20,
103,
116,
95,
37,
36,
39,
32,
28,
114,
10,
112,
111,
1,
0,
9
];
a = [122,
74,
119,
118,
149,
54,
67,
50,
46,
96,
102,
87,
160,
24,
58,
53,
64,
66,
6,
92,
42,
38,
166,
34,
21,
128,
133,
78,
159,
124,
51,
165,
125,
35,
27,
167,
57,
162,
109,
130,
52,
22,
141,
79,
132,
101,
139,
59,
134,
155,
120,
156,
56,
80,
68,
4,
105,
143,
161,
7,
65,
13,
90,
148,
73,
77,
163,
18,
40,
49,
93,
47,
88,
97,
91,
144,
30,
14,
153,
164,
131,
15,
86,
69,
127,
84,
16,
154,
115,
61,
146,
140,
110,
126,
3,
82,
48,
99,
138,
142,
63,
43,
71,
81,
147,
123,
23,
106,
158,
150,
55,
31,
152,
2,
25,
145,
76,
157,
104,
44,
117,
98,
83,
129,
94,
107,
70,
72,
75,
41,
45,
89,
60,
137,
29,
17,
100,
26,
12,
136,
11,
62,
85,
108,
113,
135,
121,
33,
5,
8,
19,
151,
20,
103,
116,
95,
37,
36,
39,
32,
28,
114,
10,
112,
111,
1,
0,
9
]
A = lables(a)
A = labels(a)
A
labels(122)
labels(74)
gg1 = [11117,
11124,
11145,
11170,
11173,
12107,
12115,
12125,
12127,
12133,
12139,
12144,
12170,
12171
]
gg2 = [10,
11,
12,
13,
17,
18,
26,
28,
49,
50,
51,
52,
53,
54,
58,
60,
11103,
11104,
11108,
11109,
11110,
11121,
11123,
11126,
11127,
11128,
11129,
11130,
11131,
11132,
11133,
11134,
11135,
11136,
11137,
11138,
11141,
11144,
11146,
11147,
11149,
11150,
11151,
11157,
11161,
11162,
11164,
11167,
11168,
11172,
11174,
12101,
12103,
12104,
12105,
12106,
12108,
12109,
12110,
12112,
12113,
12114,
12117,
12118,
12123,
12124,
12126,
12128,
12129,
12130,
12131,
12132,
12135,
12136,
12141,
12146,
12147,
12148,
12149,
12150,
12153,
12154,
12157,
12163,
12164,
12165,
12167,
12168,
12169,
12172,
12175
]
gg3 =[8,
47,
11101,
11102,
11106,
11107,
11111,
11112,
11113,
11114,
11115,
11116,
11119,
11120,
11122,
11125,
11139,
11140,
11142,
11143,
11148,
11152,
11153,
11154,
11155,
11156,
11158,
11159,
11160,
11163,
11166,
11169,
11171,
11175,
12102,
12111,
12116,
12119,
12120,
12121,
12122,
12137,
12138,
12140,
12142,
12143,
12145,
12151,
12152,
12155,
12156,
12158,
12159,
12160,
12161,
12162,
12166,
12173,
12174
];
color_mask
fMRI = nii_tool('load','aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz');
img = fMRI.img;
mask = zeros(91,109,91);
%regions = [28,60,11109,11112,11116,11131,11137,12106,12107,12129,12138,12168,12170,12174];
%regions = [11101,11106,11116,11118,11121,11124,11125,11129,11130,11135,11138,11141,11148,11150,11156,11161,11165,11166,11171,11172,11173,11174,12107,12110,12115,12116,12125,12136,12137,12138,12151,12153,12154,12155,12156,12157,12161,12162,12168,12172,12173,12174];
regions = [12153,12169,12116,12126];
for i = 1:length(regions)
mask(img==regions(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_th0.05_middle.nii');
regions=[0,   9,  19,  28,  29,  31,  32,  33,  36,  37,  39,  60,  62,
69,  70,  71,  72,  75,  76,  77,  83,  86,  94, 103, 111, 112,
113, 114, 135, 137, 144, 150, 151, 152, 158
];
regions=[0,
9,
19,
28,
29,
31,
32,
33,
36,
37,
39,
60,
62,
69,
70,
71,
72,
75,
76,
77,
83,
86,
94,
103,
111,
112,
113,
114,
135,
137,
144,
150,
151,
152,
158
];
for i = 1:length(regions)
mask(img==regions(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_th0.05_middle.nii');
fMRI = nii_tool('load','aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz');
img = fMRI.img;
mask = zeros(91,109,91);
for i = 1:length(regions)
mask(img==regions(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_th0.05_middle.nii');
fMRI = nii_tool('load','aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz');
img = fMRI.img;
mask = zeros(91,109,91);
for i = 1:length(regions)
mask(img==labels(regions(i)))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_th0.05_middle.nii');
labels[0]
labels(0)
labels00)
labels(1)
for i = 1:length(regions)
mask(img==labels(regions(i)+1))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_th0.05_middle.nii');
g_ins1 = intrsect(group1,g1);
g_ins1 = intersect(group1,g1);
g_ins2 = intersect(group33,g2);
g_ins3 = intersect(group22,g3);
fMRI = nii_tool('load','aparc.a2009s+aseg-reorient-mni152_2mm_flirt_12.mtx.nii.gz');
img = fMRI.img;
mask = zeros(91,109,91);
%regions = [28,60,11109,11112,11116,11131,11137,12106,12107,12129,12138,12168,12170,12174];
%regions = [11101,11106,11116,11118,11121,11124,11125,11129,11130,11135,11138,11141,11148,11150,11156,11161,11165,11166,11171,11172,11173,11174,12107,12110,12115,12116,12125,12136,12137,12138,12151,12153,12154,12155,12156,12157,12161,12162,12168,12172,12173,12174];
regions = [12153,12169,12116,12126];
for i = 1:length(g_ins1)
mask(img==g_ins1(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_ins_g1.nii');
mask = zeros(91,109,91);
for i = 1:length(g_ins2)
mask(img==g_ins2(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_ins_g2.nii');
mask = zeros(91,109,91);
for i = 1:length(g_ins3)
mask(img==g_ins3(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'binary_test0_ins_g3.nii');
%-- 12/05/2017 02:10:16 PM --%
load('/media/xiaoxiao/Basket III/sde/Data/Biopoint/MAT/ProcessedData/controlchild.mat')
load('/media/xiaoxiao/Basket III/sde/Data/Biopoint/MAT/controlfMRI.mat')
%-- 12/12/2017 04:10:20 PM --%
group1=[11101,
11106,
11116,
11118,
11121,
11124,
11125,
11129,
11130,
11135,
11138,
11141,
11148,
11150,
11156,
11161,
11165,
11166,
11171,
11172,
11173,
11174,
12107,
12110,
12115,
12116,
12125,
12136,
12137,
12138,
12151,
12153,
12154,
12155,
12156,
12157,
12161,
12162,
12168,
12172,
12173,
12174
]
group2=[8,
47,
11101,
11102,
11105,
11106,
11107,
11111,
11112,
11113,
11114,
11115,
11116,
11118,
11119,
11120,
11121,
11122,
11125,
11126,
11127,
11128,
11136,
11139,
11140,
11143,
11145,
11148,
11152,
11153,
11154,
11155,
11157,
11158,
11159,
11160,
11162,
11163,
11165,
11166,
11168,
11169,
12102,
12111,
12116,
12119,
12120,
12121,
12122,
12125,
12126,
12127,
12130,
12137,
12138,
12143,
12145,
12151,
12152,
12157,
12158,
12159,
12160,
12161,
12162,
12166,
12173,
12174
]
group3=[10,
11,
12,
13,
17,
18,
26,
28,
49,
50,
51,
52,
53,
54,
58,
60,
11101,
11103,
11104,
11105,
11108,
11109,
11110,
11117,
11121,
11123,
11125,
11126,
11127,
11128,
11129,
11130,
11131,
11132,
11133,
11134,
11135,
11136,
11137,
11138,
11141,
11144,
11146,
11147,
11149,
11150,
11151,
11156,
11157,
11161,
11162,
11164,
11167,
11168,
11170,
11171,
11172,
11173,
11174,
11175,
12101,
12103,
12104,
12105,
12106,
12107,
12108,
12109,
12110,
12112,
12113,
12114,
12115,
12117,
12118,
12123,
12124,
12126,
12127,
12128,
12129,
12130,
12131,
12132,
12133,
12134,
12135,
12136,
12139,
12140,
12141,
12144,
12146,
12147,
12148,
12149,
12150,
12151,
12153,
12154,
12156,
12157,
12163,
12164,
12165,
12167,
12168,
12169,
12170,
12171,
12172,
12175
]
group33=[10,
11,
12,
13,
17,
18,
26,
28,
49,
50,
51,
52,
53,
54,
58,
60,
11103,
11104,
11108,
11109,
11110,
11117,
11123,
11131,
11132,
11133,
11134,
11137,
11144,
11146,
11147,
11149,
11151,
11164,
11167,
11170,
11175,
12101,
12103,
12104,
12105,
12106,
12108,
12109,
12112,
12113,
12114,
12117,
12118,
12123,
12124,
12128,
12129,
12131,
12132,
12133,
12134,
12135,
12139,
12140,
12141,
12144,
12146,
12147,
12148,
12149,
12150,
12163,
12164,
12165,
12167,
12169,
12170,
12171,
12175
]
group22=[8,
47,
11102,
11105,
11107,
11111,
11112,
11113,
11114,
11115,
11119,
11120,
11122,
11126,
11127,
11128,
11136,
11139,
11140,
11143,
11145,
11152,
11153,
11154,
11155,
11157,
11158,
11159,
11160,
11162,
11163,
11168,
11169,
12102,
12111,
12119,
12120,
12121,
12122,
12126,
12127,
12130,
12143,
12145,
12152,
12158,
12159,
12160,
12166
]
group22=[8,
group22=[8,
g1=[11105,
11117,
11124,
11127,
11128,
11129,
11139,
11157,
11165,
11166,
12106,
12113,
12120,
12125,
12126,
12127,
12143,
12148,
12151,
12157,
];
11117,
g2=[8,
47,
52,
11107,
11109,
11110,
11126,
11141,
11146,
11147,
11167,
11168,
11172,
11175,
12103,
12104,
12108,
12109,
12110,
12112,
12116,
12117,
12128,
12129,
12133,
12138,
12139,
12140,
12146,
12154,
12156,
12163,
12167,
12169,
12171,
12172,
12175
]
g3=[10,
11,
17,
18,
28,
49,
53,
54,
11101,
11102,
11106,
11111,
11112,
11113,
11114,
11119,
11120,
11121,
11122,
11125,
11131,
11132,
11134,
11135,
11137,
11138,
11143,
11144,
11145,
11148,
11149,
11150,
11152,
11153,
11154,
11155,
11158,
11159,
11160,
11162,
11163,
11169,
11170,
12101,
12102,
12105,
12107,
12111,
12114,
12119,
12121,
12122,
12123,
12124,
12131,
12135,
12137,
12141,
12144,
12145,
12149,
12152,
12153,
12158,
12159,
12160,
12161,
12165,
12166,
12170,
12173,
12174
];
g_ins1 = intersect(group1,g1);
g_ins2 = intersect(group33,g2);
g_ins3 = intersect(group22,g3);
%-- 01/16/2018 12:50:21 PM --%
read_ABIDE
fid = fopen(subj_list,'rt');
fid = fopen(badsubj_list,'rt');
badsubj = textscan(fid,'%s','Delimiter','\n');
read_ABIDE
s =1
subj = subjects{s};
display(['Computing Correlation Matrices for Subject ',subj,' ...']);
% Subject-Native Space
display('Subject-Native Space');
% Load Data
idata = load_nifti([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.vol;
idata = load_nifti([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.vol;
idata = idata.img;
size(idata)
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.img;
sdata = load_nifti([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
sdata = load_nii([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
a=setdiff(subjects,badsubj);
read_ABIDE
[save_dir,subj,'_downsample','.h5']
%-- 01/19/2018 09:28:09 AM --%
read_ABIDE
[save_dir,subj,'_downsample','.h5']
i = 1
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
Generate_3DfMRI_dowmsampled
subj = subjects_con{1};
clc
ckear all
clear all
Generate_3DfMRI_dowmsampled
s = 1
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,140],'ChunkSize',[sz,1]);
h5create([save_dir,subjects_con{s},'_downsample','.h5'],'/fMRI',[sz,140],'ChunkSize',[sz,1]);
read_ABIDE
h5create([save_dir,subj,'_downsample'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4));
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)]);
h5create('test.h5','/fMRI',[sz,imsize(4)]);
read_ABIDE
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
[save_dir,subj,'_downsample','.h5']
read_ABIDE
for s = 42:95
subj = subjects{s};
display(['Computing Correlation Matrices for Subject ',subj,' ...']);
% Subject-Native Space
display('Subject-Native Space');
% Load Data
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.img;
sdata = load_nii([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
sdata = sdata.img;
imsize = size(idata);
%fMRI = zeros([sz,imsize(4)]);
indicator = 0; % indicate if it's control
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create([save_dir,subj,'_downsample','.h5'],'/sdata',sz);
h5create([save_dir,subj,'_downsample','.h5'],'/indicator',1);
for i = 1:imsize(4)
[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
imout = interp3(idata(:,:,:,i),x,y,z); % downsampled figure
h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',imout,[1,1,1,i],[sz,1]);
end
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
%
% sout = sdata(2:3:end,2:3:end,2:3:end);
%
%     %h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',idata);
h5write([save_dir,subj,'_downsample','.h5'],'/sdata',sout);
h5write([save_dir,subj,'_downsample','.h5'],'/indicator',indicator);
end
size(idata)
save('subjects.mat',subjects)
save('subjects.mat','subjects')
%-- 02/21/2018 12:13:31 PM --%
path  =  '/media/xiaoxiao/Basket III/ABIDE_Code/ho_roi_atlas.nii.gz'
sdata = load_nifti(path)
sdata = load_nifti('ho_roi_atlas.nii.gz')
sdata = sdata.vol
sz = [32 32 32];
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
h5create([save_dir,subj,'_downsample','.h5'],'/sdata',sz);
h5create('harvard_oxford_downsample.h5','/sdata',sz);
h5write('harvard_oxford_downsample.h5','/sdata',sout);
%-- 02/24/2018 11:48:38 AM --%
%sz = [32 32 17]; % desired downsample size
sz = [32 32 32];
sdata = load_nifti('aal_roi_atlas.nii.gz');
sdata = sdata.vol; % dim = 64 64 34
h5create(['aal','_downsample','.h5'],'/sdata',sz);
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
h5write('aal','_downsample','.h5'],'/sdata',sout);
h5write(['aal','_downsample','.h5'],'/sdata',sout);
%-- 02/24/2018 07:49:56 PM --%
read_ABIDE
s =1
read_ABIDE
save_dir
read_ABIDE
save_dir
read_ABIDE
imout = interp3(idata(:,:,:,i),x,y,z);
imshow(imout(16,:,:))
imagesc(imout(16,:,:))
imagesc(squeeze(imout(16,:,:)))
shape(idata)
size(idata)
imagesc(squeeze(squeeze(idata(32,:,:,1)))
imagesc(squeeze(squeeze(idata(32,:,:,1))))
imagesc(squeeze(sdata(32,:,:)))
imagesc(squeeze(squeeze(idata(32,:,:,100))))
imshow(squeeze(squeeze(idata(32,:,:,100))))
imshow(squeeze(squeeze(idata(:,:,20,100))))
imagesc(squeeze(squeeze(idata(:,:,20,100))))
imshow(squeeze(squeeze(idata(:,:,20,100))))
imshow(squeeze(squeeze(idata(:,32,:,100))))
read_ABIDE
imagesc(squeeze(squeeze(idata(32,:,:,1))))
i=1
[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
imout = interp3(idata(:,:,:,i),x,y,z); % downsampled figure
[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
imout = interp3(idata(:,:,:,i),x,y,z);
imagesc(squeeze(squeeze(idata(32,:,:,1))))
imout = resize(idata, sz)
idata = typecast(idata,'single')
idata = single(idata)
imout = resize(idata, sz)
figure;imagesc(squeeze(imout(:,:,16)))
[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
imout = interp3(idata(:,:,:,i),x,y,z);
figure;imagesc(squeeze(imout(:,:,16)))
figure(1);figure(2)
[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
sout = interp3(sdata,x,y,z,'nearest');
figure;imagesc(squeeze(sout(:,:,16)))
sout = resize(sidata, sz, 'nearest')
sout = resize(sdata, sz, 'nearest');
figure;imagesc(squeeze(sout(:,:,16)))
read_ABIDE
size(idata)
read_ABIDE
for s = 42:95
subj = subjects{s};
display(['Computing Correlation Matrices for Subject ',subj,' ...']);
% Subject-Native Space
display('Subject-Native Space');
% Load Data
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.img;
sdata = load_nii([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
sdata = sdata.img;
imsize = size(idata);
%fMRI = zeros([sz,imsize(4)]);
indicator = 0; % indicate if it's control
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create([save_dir,subj,'_downsample','.h5'],'/sdata',sz);
h5create([save_dir,subj,'_downsample','.h5'],'/indicator',1);
for i = 1:imsize(4)
%[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
%imout = interp3(idata(:,:,:,i),x,y,z); % downsampled figure
imout = resize(idata(:,:,:,i),sz);
h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',imout,[1,1,1,i],[sz,1]);
end
%[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
%sout = interp3(sdata,x,y,z,'nearest');
sout = resize(sidata, sz, 'nearest')
%
% sout = sdata(2:3:end,2:3:end,2:3:end);
%
%     %h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',idata);
h5write([save_dir,subj,'_downsample','.h5'],'/sdata',sout);
h5write([save_dir,subj,'_downsample','.h5'],'/indicator',indicator);
end
for s = 42:95
subj = subjects{s};
display(['Computing Correlation Matrices for Subject ',subj,' ...']);
% Subject-Native Space
display('Subject-Native Space');
% Load Data
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-smooth5-bptf_l0.01Hz.h0.1Hz-resid.nii.gz']);
idata = idata.img;
sdata = load_nii([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
sdata = sdata.img;
imsize = size(idata);
%fMRI = zeros([sz,imsize(4)]);
indicator = 0; % indicate if it's control
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create([save_dir,subj,'_downsample','.h5'],'/sdata',sz);
h5create([save_dir,subj,'_downsample','.h5'],'/indicator',1);
for i = 1:imsize(4)
%[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
%imout = interp3(idata(:,:,:,i),x,y,z); % downsampled figure
imout = resize(idata(:,:,:,i),sz);
h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',imout,[1,1,1,i],[sz,1]);
end
%[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
%sout = interp3(sdata,x,y,z,'nearest');
sout = resize(sdata, sz, 'nearest')
%
% sout = sdata(2:3:end,2:3:end,2:3:end);
%
%     %h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',idata);
h5write([save_dir,subj,'_downsample','.h5'],'/sdata',sout);
h5write([save_dir,subj,'_downsample','.h5'],'/indicator',indicator);
end
figure;imagesc(squeeze(imout(:,:,16)))
figure;imagesc(squeeze(imout(16,:,:)))
figure;imagesc(squeeze(squeeze(idata(32,:,:,293))))
subjects{42}
for s = 42:95
subj = subjects{s};
display(['Computing Correlation Matrices for Subject ',subj,' ...']);
% Subject-Native Space
display('Subject-Native Space');
% Load Data
idata = load_nii([data_dir,subj,'/rsfMRI/rsfMRI-reorient-skip7-mc_mid-brain-stc-mni152_2mm_fnirt.nii.gz']);
idata = idata.img;
sdata = load_nii([data_dir,subj,'/rsfMRI/anat-reorient/anat2rsfMRI/',seg_name,'-reorient_',suff,'.mtx.nii.gz']);
sdata = sdata.img;
imsize = size(idata);
%fMRI = zeros([sz,imsize(4)]);
indicator = 0; % indicate if it's control
h5create([save_dir,subj,'_downsample','.h5'],'/fMRI',[sz,imsize(4)],'ChunkSize',[sz,1]);
h5create([save_dir,subj,'_downsample','.h5'],'/sdata',sz);
h5create([save_dir,subj,'_downsample','.h5'],'/indicator',1);
for i = 1:imsize(4)
%[y,x,z]=ndgrid(linspace(1,size(idata(:,:,:,i),1),sz(1)),linspace(1,size(idata(:,:,:,i),2),sz(2)),linspace(1,size(idata(:,:,:,i),3),sz(3)));
%imout = interp3(idata(:,:,:,i),x,y,z); % downsampled figure
imout = resize(idata(:,:,:,i),sz);
h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',imout,[1,1,1,i],[sz,1]);
end
%[y,x,z]=ndgrid(linspace(1,size(sdata,1),sz(1)),linspace(1,size(sdata,2),sz(2)),linspace(1,size(sdata,3),sz(3)));
%sout = interp3(sdata,x,y,z,'nearest');
sout = resize(sdata, sz, 'nearest');
%
% sout = sdata(2:3:end,2:3:end,2:3:end);
%
%     %h5write([save_dir,subj,'_downsample','.h5'],'/fMRI',idata);
h5write([save_dir,subj,'_downsample','.h5'],'/sdata',sout);
h5write([save_dir,subj,'_downsample','.h5'],'/indicator',indicator);
end
figure;imagesc(squeeze(imout(16,:,:)))
read_ABIDE_NYU
save('subjects_nyu.mat','subjects')
regions =[6401.0,
4102.0,
2311.0,
2312.0,
8201.0,
8202.0,
4111.0,
2322.0,
8212.0,
2601.0,
2602.0,
2611.0,
2612.0,
2101.0,
2102.0,
7001.0,
7002.0,
2401.0,
2402.0,
7011.0,
7012.0,
8301.0,
2201.0,
2202.0,
4001.0,
4002.0,
8111.0,
8112.0,
9140.0,
8122.0,
3002.0,
3001.0,
2001.0,
2002.0,
2302.0
]
color_mask
mask = zeros(65,77,63);
for i = 1:length(regions)
mask(img==regions(i))=1;
end
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_blackout_1.nii');
sz = [91,109,91]
mask = resize(mask,sz)
nii_tool('save',nii,'ABIDE_blackout_1.nii');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_blackout_1.nii');
regions = [25, 28, 30, 62, 69, 72, 77, 84, 88]
regions=[6202.0, 6211.0, 6221.0, 9120.0, 9130.0, 8111.0, 4021.0, 9150.0, 9160.0
]
mask = zeros(65,77,63)
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest')
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_sample.nii');
for i = 0:31
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
%newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
end
close all
for i = 0:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
%origim= nii_tool('img',strcat('output_oversub/pat',int2str(i),'.nii'));
%newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[16 16 1 16]),'displayrange',[0 0.01])
end
close all
for i = 0:31
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32]))
end
close all
for i = 0:31
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32],'displayrange',[-0.005 0.005]))
end
for i = 0:31
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[-0.005 0.005])
end
close all
for i = 0:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 16]),'displayrange',[-0.005 0.005])
end
for i = 0:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
end
close all
regions = [0, 2, 9, 13, 16, 28, 38, 55, 63, 76, 77, 85, 88, 91, 97, 101, 103, 104, 105
]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest')
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_s&b_1.nii');
regions=[6401.,  4101.,  4112.,  8212.,  2331.,  6201.,  6221.,  4202.,
6002.,  6301.,  6302.,  8101.,  4011.,  8112.,  8121.,  7101.,
7102.,  2501.,  2502.
];
regions =[6401.,  4101.,  4112.,  8212.,  2331.,  6201.,  6221.,  4202.,
6002.,  6301.,  6302.,  8101.,  4011.,  8112.,  8121.,  7101.,
7102.,  2501.,  2502.
]
regions =[6401.,  4101.,  4112.,  8212.,  2331.,  6201.,  6221.,  4202.,
6002.,  6301.,  6302.,  8101.,  4011.,  8112.,  8121.,  7101.,
7102.,  2501.,  2502.]
regions =[6401.,  4101.,  4112.,  8212.,  2331.,  6201.,  6221.,  4202., 6002.,  6301.,  6302.,  8101.,  4011.,  8112.,  8121.,  7101., 7102.,  2501.,  2502.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_s&b_1.nii');
regions = [ 2501.  2502.  8101.  6302.  6221.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both_1.nii');
regions = [ 2311.  2312.  2321.  2322.  2601.  2602.  9002.  2611.  2612.  2101.
2102.  9011.  9012.  2111.  2112.  5201.  5202.  9051.  9052.  2402.
9062.  5001.  5002.  2701.  2702.  5011.  5012.  2201.  2202.  5021.
5022.  4001.  2211.  2212.  4002.  5301. ]
regions = [ 2311.  2312.  2321.  2322.  2601.  2602.  9002.  2611.  2612.  2101. 2102.  9011.  9012.  2111.  2112.  5201.  5202.  9051.  9052.  2402. 9062.  5001.  5002.  2701.  2702.  5011.  5012.  2201.  2202.  5021. 5022.  4001.  2211.  2212.  4002.  5301. ]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con_1.nii');
regions = [[ 6401.  4101.  4102.  8201.  8202.  4111.  4112.  8211.  8212.  5401. 5402.  2331.  6201.  6202.  9021.  9022.  6211.  6212.  9031.  9032. 9041.  9042.  4201.  4202.  8301.  8302.  7021.  7022.  9071.  9072. 6002.  9081.  9082.  9100.  9110.  6301. ]
]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat_1.nii');
regions = [ 6202.,  6211.,  6221.,  9120.,  8101.,  8111.,  4021.,  9150.,
9160.]
regions = [ 6202.,  6211.,  6221.,  9120.,  8101.,  8111.,  4021.,  9150., 9160.0]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both_2.nii');
regions = [[ 6401.  8121.  4101.  7101.  7102.  2501.  4112.  2502.  6301.  8212. 6302.  2331.  8101.  4202.  4011.  8112.  6201.  6002.]]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both_2.nii');
regions = [ 6402.  2312.  2321.  2322.  2332.  9001.  9011.  2111.  2112.  5201. 5202.  7001.  7002.  2401.  2402.  7011.  7012.  9062.  6001.  5002. 2701.  2702.  5011.  2211.  2212.  4012.  5301.  8122.  3002.  3001. 2001.  2002.  5101.  5102.  2301.  2302.];
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con_2.nii');
regions = [ 4102.  8201.  8202.  4111.  5401.  6202.  9021.  9022.  6211.  6212. 9031.  9032.  6222.  9041.  9042.  8301.  8302.  7021.  7022.  9071. 9072.  9100.  9110.  9120.  8102.  8111.  4021.  4022.  9170.  6101. 6102.];
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat_2.nii');
regions = [[ 2001.  9170.  6102.]]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_both.nii');
regions = [ 6211.  8201.  6302.  8212.  5401.  2331.  4201.  9140.  6001.  9022.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_con.nii');
regions=[ 6222.  5102.  2211.  9001.  9002.  9062.  8112.  9072.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_pat.nii');
regions = 2111.,  8121.,  6211.,  6222.,  2001.,  9170.,  6302.,  5401.,
6102.,  2331.,  2211.,  9001.,  9002.,  9062.,  4201.,  9072.,
6001.,  9022.
regions = [2111.,  8121.,  6211.,  6222.,  2001.,  9170.,  6302.,  5401.,
6102.,  2331.,  2211.,  9001.,  9002.,  9062.,  4201.,  9072.,
6001.,  9022.
]
regions = [2111.,  8121.,  6211.,  6222.,  2001.,  9170.,  6302.,  5401., 6102.,  2331.,  2211.,  9001.,  9002.,  9062.,  4201.,  9072., 6001.,  9022.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_sample.nii');
regions = [ 9001.  9002.  6222.  9062.  9072.  6302.  8121.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_both2.nii');
regions = [ 2322.  6212.  6301.  2002.  5102.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_pat2.nii');
regions = [ 8202.  2321.  5402.  2602.  2101.  9011.  6221.  5201.  5202.  9042. 9051.  9052.  2401.  2402.  9061.  8302.  9071.  9082.  5001.  5002. 5011.  5012.  2201.  5021.  5022.  9130.  9140.  5301.  5302.  9160. 5101.  2301.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_con2.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_con2_aal.nii');
regions = [ 2322.  6212.  6301.  2002.  5102.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_pat2_aal.nii');
regions = [ 9001.  9002.  6222.  9062.  9072.  6302.  8121.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'BIO_both2_aal.nii');
regions = [ 4101.  2331.  2332.  6201.  7001.  4202.  2701.  6301.  5021.  8101. 8102.  4011.  8112.  3001.  7101.  7102.  2501.  2502.  9160.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both3.nii');
regions = [ 8202.  8211.  6202.  6222.  9041.  9042.  8301.  8302.  7021.  9072. 9082.  9100.  4021.  4022.  6101.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat3.nii');
regions = [ 9001.  2612.  2102.  5002.  2702.  5102.  2301.  2302.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con3.nii');
sz2 = [65,77,63]
MRI = nii_tool('load','MNI152_T1_2mm_brain.nii.gz');
img = MRI.img;
img_new = resize(image,sz2);
nii = nii_tool('init',img_new);
nii_tool('save',nii,'MNI152_T1_2mm_brain_downsample.nii');
sz2 = [65,77,63]
MRI = nii_tool('load','MNI152_T1_2mm_brain.nii.gz');
img = MRI.img;
img_new = resize(img,sz2);
nii = nii_tool('init',img_new);
nii_tool('save',nii,'MNI152_T1_2mm_brain_downsample.nii');
sz2 = [65,77,63]
MRI = nii_tool('load','MNI152_T1_2mm_brain.nii.gz');
img = single(MRI.img);
img_new = resize(img,sz2);
nii = nii_tool('init',img_new);
nii_tool('save',nii,'MNI152_T1_2mm_brain_downsample.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con3_aal.nii');
fMRI = nii_tool('load','aal_roi_atlas.nii.gz');
img = fMRI.img;
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con3_aal.nii');
regions = [ 8202.  8211.  6202.  6222.  9041.  9042.  8301.  8302.  7021.  9072. 9082.  9100.  4021.  4022.  6101.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat3_aal.nii');
regions = [ 4101.  2331.  2332.  6201.  7001.  4202.  2701.  6301.  5021.  8101. 8102.  4011.  8112.  3001.  7101.  7102.  2501.  2502.  9160.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both3_aal.nii');
for i = 0:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
end
close all
i = 0;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
temp = newim-newim2;
for i = 1:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
%figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
temp = temp + newim-newim2;
end
figure(); montage(reshape(temp/64,[16 16 1 16]),'displayrange',[-0.005 0.005])
figure(); montage(reshape(temp/64,[16 16 1 16]),'displayrange',[-0.002 0.002])
regions = [ 8101.  9160.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both4.nii');
regions = [ 6202.  6211.  9120.  8111.  4021.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat4.nii');
regions = [ 6221.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con4.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con4_aal.nii');
regions = [ 6202.  6211.  9120.  8111.  4021.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat4_aal.nii');
regions = [ 8101.  9160.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both4_aal.nii');
for i = 0:63
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
%temp = temp + newim-newim2;
end
close all
figure(); montage(reshape(newim-newim2,[16 1 16 16]),'displayrange',[-0.005 0.005])
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con2_',int2str(i),'.nii'));
newim= flipud(permute(origim,[3 2 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat2_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[3 2 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
i = 0;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con1_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat1_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
i = 0;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim-newim2,[16 16 1 16]),'displayrange',[-0.005 0.005])
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[-0.005 0.005])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[-0.005 0.005])
i =4;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim-newim2,[32 32 1 32]),'displayrange',[-0.005 0.005])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.005])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
i =10;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
i =6;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
i =11;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
i =15;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
temp = newim-newim2;
i =14;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
temp = newim-newim2;
for i = 0:31
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim= flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
%figure;imagesc(squeeze(newim(:,16,:)),[0, 0.03])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.01])
%temp = temp + newim-newim2;
end
class all
close all
i =30;
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/con_',int2str(i),'.nii'));
newim = flipud(permute(origim,[2 3 1]));
origim= nii_tool('img',strcat('/media/xiaoxiao/Basket III/ABIDE_Code/middle_outputs/pat_',int2str(i),'.nii'));
newim2= flipud(permute(origim,[2 3 1]));
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.05])
figure(); montage(reshape(newim,[32 32 1 32]),'displayrange',[0 0.02])
regions = [ 2331.  6201.  7012.  4202.  2701.  6302.  8102.  8112.  8122.  3002. 3001.  7102.  9160.  9170.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both5_aal.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_both5.nii');
regions = [ 8202.  5402.  6202.  4201.  8301.  7022.  4022.  6102.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat5.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_pat5_aal.nii');
regions = [ 2312.  2102.  2111.  5002.  4001.]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con5_aal.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'ABIDE_con5.nii');
regions = [8121.0, 6302.0, 6222.0]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_both5.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_both5_aal.nii');
regions = [2002.0, 2322.0, 6301.0, 5102.0]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_pat5_aal.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_pat5.nii');
regions=[5001.0, 8202.0, 5002.0, 2321.0, 5011.0, 5012.0, 2201.0, 5402.0, 5021.0, 5022.0, 2602.0, 9130.0, 9140.0, 2101.0, 5301.0, 5302.0, 2111.0, 9160.0, 6221.0, 5201.0, 5202.0, 2401.0, 2402.0, 5101.0, 8302.0, 2301.0]
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_con5.nii');
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_con5_aal.nii');
%-- 04/16/2018 10:53:21 AM --%
x = [1825.01
2147.04
2230.03
2265.03
3462.03
3839.03
5554.03
6006.03
7154.01
7166.01
7240.01
7279.01
7344.03
7691.1
7864.03
7880.1
7936.02
7984.03
8188.02
8233.03
8234.03
8237.03
8269.03
8270.03
8291.03
8299.03
8315.03
8366.02
9001.03
9030.03
9058.03
9118.03
9194.03
9202.03
9203.03
9204.03
9208.03
9223.03
9239.03
9248.03
9253.03
9262.03
9269.03
9296.03
9304.03
9330.03
9337.03
9340.03
9345.03
9349.03
9378.03
9385.03
9397.03
9458.03
9471.03
9514.03
9515.03
9534.03
9681.03
9956.03
10023.03
10048.03
10113.03
10170.03
10244.03
10404.03
10029.03
]
x'
a  = round(a,2)
a  = round(ans,2)
a  = roundn(ans,-2)
a  = ans*100
c = a/100
c(1)
format long
c = a/100
c(1)
a = num2str(x)'
a = num2str(x)
b = a'
b = a.T
b = transpose(A)
b = transpose(a)
format short g
a = x'
x
clear
clc
female = [4383.03
7972.03
8266.04
8307.03
8311.03
8320.03
9104.03
9104.05
9239.04
9247.03
9260.03
9270.03
9350.03
9568.03
]
format double
format single
format long
female(1)
fMRI = nii_tool('load','aal_roi_atlas.nii.gz');
img = fMRI.img;
mask = zeros(65,77,63);
regions = [2311., 8202., 2601., 2602., 2101., 5201., 5002., 5011., 5012.,
2201., 5021., 9130., 9140., 9150., 9160., 9170., 5101., 2301.
]
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_both_aal.nii');
regions = [[5402., 5202., 2401., 5001., 5301., 5302., 5102.]
];
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_girls_aal.nii');
regions = [8201., 6221., 6222., 2402., 2702., 2211.]
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_boys_aal.nii');
sz2 = [91,109,91]
MRI = nii_tool('load','Bio_gender_boys_aal.nii.gz');
img = single(MRI.img);
img_new = resize(img,sz2);
nii = nii_tool('init',img_new);
nii_tool('save',nii,'Bio_gender_boys_mni.nii');
img_new = resize(img,sz2);
upsampling
mask = zeros(65,77,63);
% for i = 1 : length(regions)
%     mask(img==regions(i))=1;
% end
% %mask = resize(mask,sz,'nearest');
% nii=nii_tool('init',mask);
% nii_tool('save',nii,'Bio_con5_aal.nii');
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_boys_aal.nii');
regions=[5402., 5202., 2401., 5001., 5301., 5302., 5102.]
mask = zeros(65,77,63);
% for i = 1 : length(regions)
%     mask(img==regions(i))=1;
% end
% %mask = resize(mask,sz,'nearest');
% nii=nii_tool('init',mask);
% nii_tool('save',nii,'Bio_con5_aal.nii');
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_girls_aal.nii');
regions =[2311., 8202., 2601., 2602., 2101., 5201., 5002., 5011., 5012.,
2201., 5021., 9130., 9140., 9150., 9160., 9170., 5101., 2301.]
;
color_mask
fMRI = nii_tool('load','aal_roi_atlas.nii.gz');
img = fMRI.img;
mask = zeros(65,77,63);
for i = 1 : length(regions)
mask(img==regions(i))=1;
end
%mask = resize(mask,sz,'nearest');
nii=nii_tool('init',mask);
nii_tool('save',nii,'Bio_gender_both_aal.nii');
upsampling

